Adaptive Batch-Wise Sample Scheduling for Direct Preference Optimization

Direct Preference Optimization (DPO) has emerged as an effective approach for aligning large language models (LLMs) with human preferences. However, its performance is highly dependent on the quality of the underlying human preference data. To address this bottleneck, prior work has explored various data selection strategies, but these methods often overlook the impact of the evolving states of the language model during the optimization process. In this paper, we introduce a novel problem: Sample Scheduling for DPO, which aims to dynamically and adaptively schedule training samples based on the model's evolving batch-wise states throughout preference optimization. To solve this problem, we propose SamS, an efficient and effective algorithm that adaptively selects samples in each training batch based on the LLM's learning feedback to maximize the potential generalization performance. Notably, without modifying the core DPO algorithm, simply integrating SamS significantly improves performance across tasks, with minimal additional computational overhead. This work points to a promising new direction for improving LLM alignment through batch-wise sample selection, with potential generalization to RLHF and broader supervised learning paradigms.

==> algorithms/practice.tex <==
\begin{algorithm}
\caption{The Practical Version of  our Adaptive Sample Scheduling algorithm}
\label{alg:practical}
\begin{algorithmic}[1]
\REQUIRE batch size $n$, batch data $X$, selected batch size $\hat{n}$, random batch pool $\mathcal{P}$, policy $\pi_{\theta_0}$, scheduler $\hat{\theta}_0$
\FOR{$t = 2, 3, \dots, T$}
    \STATE Draw batch data $X_t = \{ (x_{t,i},y_{w,t,i},y_{l,t,i})|i = 1,2,\dots,n\}\sim \mathcal{D}$ 
    \STATE \textbf{DPO Forward}: 
    \STATE Compute DPO Loss $L_{\text{DPO}}(\pi_{\theta_t}, X_t)$ 
    \STATE Get the hidden state of policy $H_t=\{h_{t,i}|i = 1,2,\dots,n\}$
    \STATE Get $A=\frac{1}{n} \sum_{i=1}^{n} e^{\mathcal{L}_{\text{DPO}}(\pi_{\theta_{t-1}}; x_{t-1,i}, y_{w,t-1,i}, y_{l,t-1,i})}  $)
    \STATE Compute $ B=\frac{1}{n} \sum_{i=1}^{n} e^{\mathcal{L}_{\text{DPO}}(\pi_{\theta_t}; x_{t,i}, y_{w,t,i}, y_{l,t,i})}$
    \STATE For $X_{t - 1}$, Compute $r^{batch}_{t - 1}=(A - B)/\max(A,B)$  
    
    % \FOR{$i = 1,2,\dots,n$}
    %     \STATE Compute $\pi_{\theta_t}(y_w|x_{t,i}), \pi_{\theta_t}(y_l|x_{t,i}), \pi_{\text{ref}}(y_w|x_{t,i}), \pi_{\text{ref}}(y_l|x_{t,i})$ 
    % \ENDFOR
    %Compute $f(h(x_{t,i}; \hat{\theta}_{t-1});\theta_{t-1})$
    \STATE \textbf{Scheduler Training}:
    \FOR{$i = 1,2,3,\dots,n$}
        \STATE Compute $\hat{r}^{sample}_{i,t - 1}$ according to Section~\ref{sec:framwork}
        \STATE Compute $r^{sample}_{t,i}= (1-\gamma) \sigma(\hat{r}^{sample}_{t,i}) + \gamma \sigma(map(r^{batch}_{t}))$
    \ENDFOR 
    \STATE Get offline train data for scheduler $T^{online}_{t - 1}=\{h_{t-1,i},r^{sample}_{i,t - 1}|i = 1,2,\dots,n\}$ 
    \STATE Randomly fetch $S$ batches $\{T_{i}^{\text{offline}}|i = 1,2,\dots,S\}$ from $P$
    \STATE Get current train data $T_{t - 1}=\{T^{online}_{t - 1},T_{1}^{\text{offline}},\dots,T_{S}^{\text{offline}}\}=\{H_{t - 1},R_{t - 1}\}$ 
    \STATE $\mathcal{L}_{\hat{\theta}_t}(H_{t - 1})=(\hat{\theta}_{t - 1}(H_{t - 1})-R_{t - 1})^2/2$ 
    \STATE $\hat{\theta}_{t}=\hat{\theta}_{t - 1}-\eta_{\theta}\nabla_{\hat{\theta}_{t - 1}}\mathcal{L}_{\hat{\theta}_{t - 1}}(H_{t - 1})$ 
    \STATE Append $T^{online}_t$ into $\mathcal{P}$ 
    \STATE \textbf{Scheduler Forward}: 
    \STATE $R_{\text{predict}}=\hat{\theta}_{t}(H_t)=\{\hat{r}_{i,t}\},i = 1,2,\dots,n$ 
    \STATE Get a distribution $D_t^{\text{Samples}}$ based on $R_{\text{predict}}$ 
    \STATE Sample $\hat{n}$ samples $\hat{X}_{t}=\{x_{i,t}\},i = 1,2,\dots,\hat{n}$ from $X_t$  
    \STATE \textbf{DPO Backward}: 
    \STATE $\pi_{\theta_{t + 1}}=\pi_{\theta_t}-\eta_{\pi}\nabla_{\pi_{\theta_t}}\mathcal{L}_{\text{DPO}}(\pi_{\theta_t}, \hat{X}_t)$
\ENDFOR
\end{algorithmic} 
\end{algorithm}





